Weakly acyclic diagrams: A data structure for infinite-state symbolic verification

Ordered binary decision diagrams (OBDDs) are a fundamental data structure for the manipulation of Boolean functions, with strong applications to finite-state symbolic model checking. OBDDs allow for efficient algorithms using top-down dynamic programming. From an automata-theoretic perspective, OBDDs essentially are minimal deterministic finite automata recognizing languages whose words have a fixed length (the arity of the Boolean function). We introduce weakly acyclic diagrams (WADs), a generalization of OBDDs that maintains their algorithmic advantages, but can also represent infinite languages. We develop the theory of WADs and show that they can be used for symbolic model checking of various models of infinite-state systems.

==> tab-petri.tex <==
\small
\begin{longtable}{lrr}
\toprule
& \wadl & \mist \\
\midrule
\texttt{peterson.spec} & 0.24 & 0.03 \\
\texttt{newdekker.spec} & 1.94 & 0.11 \\
\texttt{newrtp.spec} & 0.05 & 0.01 \\
\texttt{lamport.spec} & 0.08 & 0.02 \\
\texttt{read-write.spec} & 0.48 & 0.10 \\
\texttt{kanban.spec} & 14.99 & 599.00 \\
\texttt{fms.spec} & 1.25 & 0.06 \\
\texttt{bingham\_h250\_attic.spec} & 207.06 & 27.36 \\
\texttt{basicME.spec} & 0.02 & 0.01 \\
\texttt{pingpong.spec} & 0.03 & 0.01 \\
\texttt{csm.spec} & 0.23 & 0.04 \\
\texttt{pncsasemiliv.spec} & 15.14 & 2.51 \\
\texttt{bingham\_h50.spec} & 26.43 & 8.80 \\
\texttt{mesh2x2.spec} & 1.32 & 0.28 \\
\texttt{leabasicapproach.spec} & 0.10 & 0.01 \\
\texttt{manufacturing.spec} & 7.38 & 2.62 \\
\texttt{MultiME.spec} & 0.10 & 0.01 \\
\texttt{mesh3x2.spec} & 8.37 & 3.79 \\
\texttt{bingham\_h25.spec} & 3.85 & 0.49 \\
\texttt{multipool.spec} & 0.46 & 0.81 \\
\texttt{pncsacover.spec} & 305.63 & 599.44 \\
\texttt{extendedread-write-smallconsts.spec} & 41.82 & 426.02 \\
\texttt{kanban.spec} & 18.90 & 599.58 \\
\texttt{fms\_attic.spec} & 38.73 & 2.57 \\
\texttt{x0\_MORE\_INFO\_q5.spec} & 1180.36 & 599.65 \\
\texttt{x0\_MUST\_FIX\_q5.spec} & 1199.40 & 0.30 \\
\texttt{x0\_CLOSED\_q3.spec} & 1200.69 & 599.28 \\
\texttt{x0\_MUST\_FIX\_q1.spec} & 1199.21 & 0.18 \\
\texttt{x0\_CLOSED\_q5.spec} & 1189.56 & 0.28 \\
\texttt{x0\_MORE\_INFO\_q8.spec} & 1169.93 & 599.71 \\
\texttt{x0\_FIX\_AGAIN\_q1.spec} & 1193.17 & 4.21 \\
\texttt{x0\_MUST\_FIX\_q3.spec} & 1201.17 & 599.78 \\
\texttt{x0\_VERIFIED\_q3.spec} & 1201.21 & 599.75 \\
\texttt{x0\_PENDING\_q5.spec} & 1200.84 & 599.77 \\
\texttt{x0\_VERIFIED\_q6.spec} & 1201.18 & 2.43 \\
\texttt{x0\_PENDING\_q3.spec} & 1194.86 & 599.93 \\
\texttt{x0\_VERIFIED\_q5.spec} & 1201.03 & 0.19 \\
\texttt{x0\_PENDING\_q6.spec} & 1201.02 & 599.80 \\
\texttt{x0\_BUG\_REPORT\_q3.spec} & 1200.89 & 1.41 \\
\texttt{x0\_FIX\_AGAIN\_q5.spec} & 1201.06 & 2.01 \\
\texttt{x0\_MORE\_INFO\_q3.spec} & 1201.03 & 13.56 \\
\texttt{x0\_CLOSED\_q1.spec} & 1201.11 & 600.31 \\
\texttt{x0\_PENDING\_q8.spec} & 1197.62 & 599.72 \\
\texttt{x0\_VERIFIED\_q1.spec} & 1197.53 & 0.29 \\
\texttt{x0\_MORE\_INFO\_q6.spec} & 1201.03 & 451.45 \\
\texttt{x0\_FIXED\_q1.spec} & 1201.16 & 0.17 \\
\texttt{x0\_MUST\_FIX\_q8.spec} & 1201.14 & 2.39 \\
\texttt{x0\_PENDING\_q3\_buggy.spec} & 1199.80 & 0.82 \\
\texttt{x0\_FIXED\_q6.spec} & 1201.19 & 599.74 \\
\texttt{x0\_MORE\_INFO\_q1.spec} & 1200.67 & 599.74 \\
\texttt{x0\_PENDING\_q1.spec} & 1200.75 & 599.77 \\
\texttt{x0\_CLOSED\_q6.spec} & 1201.09 & 599.92 \\
\texttt{x0\_VERIFIED\_q8.spec} & 1201.02 & 296.74 \\
\texttt{x0\_MUST\_FIX\_q6.spec} & 1201.12 & 599.73 \\
\texttt{x0\_FIXED\_q3.spec} & 1201.19 & 0.51 \\
\texttt{x0\_FIXED\_q8.spec} & 1201.12 & 599.74 \\
\texttt{x0\_CLOSED\_q8.spec} & 1201.35 & 92.05 \\
\texttt{x0\_BUG\_REPORT\_q5.spec} & 1201.10 & 599.72 \\
\texttt{x0\_BUG\_REPORT\_q8.spec} & 1201.10 & 0.91 \\
\texttt{x0\_FIX\_AGAIN\_q3.spec} & 1201.16 & 5.91 \\
\texttt{x0\_BUG\_REPORT\_q6.spec} & 1201.09 & 31.47 \\
\texttt{x0\_BUG\_REPORT\_q1.spec} & 1201.11 & 429.44 \\
\texttt{x0\_FIX\_AGAIN\_q8.spec} & 1201.21 & 599.81 \\
\texttt{x0\_FIXED\_q5.spec} & 1201.20 & 109.34 \\
\texttt{x0\_FIX\_AGAIN\_q6.spec} & 1201.18 & 0.04 \\
\texttt{x0\_HQ\_q1.spec} & 583.21 & 4.83 \\
\texttt{x0\_HA\_q5.spec} & 1199.77 & 599.87 \\
\texttt{x0\_HQ\_q5.spec} & 1193.92 & 0.27 \\
\texttt{x0\_HA\_q1.spec} & 479.93 & 0.01 \\
\texttt{x0\_AR\_q2.spec} & 1198.33 & 87.75 \\
\texttt{x0\_AA\_q2.spec} & 1188.83 & 14.54 \\
\texttt{x0\_AA\_q5.spec} & 1173.19 & 599.14 \\
\texttt{x0\_AA\_q1.spec} & 508.90 & 599.54 \\
\texttt{x0\_HQ\_q2.spec} & 1200.26 & 14.91 \\
\texttt{x0\_AR\_q1.spec} & 434.70 & 599.77 \\
\texttt{x0\_AR\_q5.spec} & 1195.83 & 599.53 \\
\texttt{x0\_HA\_q2.spec} & 1200.25 & 599.81 \\
\texttt{howait\_\_all\_workers\_finished\_if\_wait\_over\_\_depth\_1.spec} & 1182.55 & 14.41 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_1\_\_depth\_2.spec} & 1200.44 & 599.75 \\
\texttt{stutter\_\_we\_abhorr\_as\_\_depth\_1.spec} & 96.89 & 13.42 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_3\_\_depth\_2.spec} & 1198.74 & 599.79 \\
\texttt{state\_factory\_\_single\_message\_in\_mailbox\_\_depth\_0.spec} & 1200.60 & 599.83 \\
\texttt{pipe\_\_single\_message\_in\_mailbox\_\_depth\_2.spec} & 1189.03 & 599.17 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_2\_\_depth\_1.spec} & 1179.96 & 599.36 \\
\texttt{stutter\_\_we\_abhorr\_as\_\_depth\_2.spec} & 98.96 & 67.76 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_1\_\_depth\_1.spec} & 1197.45 & 599.43 \\
\texttt{sieve\_\_single\_message\_in\_filter\_mailbox\_\_depth\_0.spec} & 1201.24 & 599.74 \\
\texttt{parikh\_\_should\_already\_be\_initialized\_\_depth\_1.spec} & 1201.33 & 599.75 \\
\texttt{concdb\_\_single\_client\_writes\_\_depth\_0.spec} & 1200.71 & 599.67 \\
\texttt{parikh\_\_should\_already\_be\_initialized\_\_depth\_2.spec} & 1201.39 & 62.86 \\
\texttt{state\_factory\_\_single\_message\_in\_mailbox\_\_depth\_1.spec} & 516.58 & 599.74 \\
\texttt{stutter\_\_we\_abhorr\_as\_\_depth\_0.spec} & 11.43 & 599.71 \\
\texttt{sieve\_\_single\_message\_in\_sieve\_mailbox\_\_depth\_0.spec} & 1201.05 & 599.82 \\
\texttt{howait\_\_all\_workers\_finished\_if\_wait\_over\_\_depth\_2.spec} & 1200.51 & 599.80 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_\_depth\_0.spec} & 1200.98 & 599.84 \\
\texttt{reslock\_\_critical\_\_depth\_1.spec} & 1200.94 & 0.09 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_3\_\_depth\_1.spec} & 1201.29 & 2.74 \\
\texttt{reslock\_\_critical\_\_depth\_2.spec} & 1200.31 & 599.81 \\
\texttt{finite\_leader\_\_single\_leader\_\_depth\_2.spec} & 1200.97 & 599.91 \\
\texttt{concdb\_\_single\_client\_writes\_\_depth\_2.spec} & 1200.58 & 599.72 \\
\texttt{unsafe\_send\_\_sending\_to\_non-pid\_\_depth\_0.spec} & 1.01 & 599.77 \\
\texttt{ring\_\_single\_message\_in\_mailbox\_\_depth\_2.spec} & -1.00 & 599.78 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_4\_\_depth\_2.spec} & 1201.17 & 599.75 \\
\texttt{reslockbeh\_\_critical\_\_depth\_2.spec} & 1199.97 & 599.69 \\
\texttt{howait\_\_all\_workers\_finished\_if\_wait\_over\_\_depth\_0.spec} & 1196.16 & 0.08 \\
\texttt{sieve\_\_single\_message\_in\_counter\_mailbox\_\_depth\_2.spec} & 1151.34 & 0.14 \\
\texttt{unsafe\_send\_\_sending\_to\_non-pid\_\_depth\_1.spec} & 1.93 & 0.07 \\
\texttt{ring\_\_single\_message\_in\_mailbox\_\_depth\_0.spec} & 1193.87 & 599.72 \\
\texttt{state\_factory\_\_after\_receive\_if\_no\_mail\_\_depth\_0.spec} & 1201.00 & 0.09 \\
\texttt{pipe\_\_single\_message\_in\_mailbox\_\_depth\_1.spec} & 1200.59 & 599.79 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_4\_\_depth\_1.spec} & 1201.37 & 599.87 \\
\texttt{sieve\_\_single\_message\_in\_counter\_mailbox\_\_depth\_1.spec} & 1200.51 & 0.15 \\
\texttt{ring\_\_single\_message\_in\_mailbox\_\_depth\_1.spec} & 1197.41 & 599.78 \\
\texttt{firewall\_\_no\_pred\_called\_with\_zero\_\_depth\_0.spec} & 1195.87 & 599.80 \\
\texttt{firewall\_\_no\_pred\_called\_with\_zero\_\_depth\_1.spec} & 1195.71 & 599.85 \\
\texttt{finite\_leader\_\_single\_leader\_\_depth\_0.spec} & 1197.13 & 599.68 \\
\texttt{finite\_leader\_\_single\_leader\_\_depth\_1.spec} & 1200.96 & 599.73 \\
\texttt{reslock\_\_critical\_\_depth\_0.spec} & 1201.55 & 0.07 \\
\texttt{pipe\_\_single\_message\_in\_mailbox\_\_depth\_0.spec} & 615.87 & 599.78 \\
\texttt{unsafe\_send\_\_sending\_to\_non-pid\_\_depth\_2.spec} & 0.86 & 599.80 \\
\texttt{reslockbeh\_\_critical\_\_depth\_1.spec} & 1192.95 & 599.71 \\
\texttt{reslockbeh\_\_critical\_\_depth\_0.spec} & 1201.01 & 599.74 \\
\texttt{concdb\_\_single\_client\_writes\_\_depth\_1.spec} & 1202.13 & 599.70 \\
\texttt{parikh\_\_should\_already\_be\_initialized\_\_depth\_0.spec} & 1201.24 & 599.73 \\
\texttt{sieve\_\_single\_message\_in\_counter\_mailbox\_\_depth\_0.spec} & 1201.23 & 0.13 \\
\texttt{safe\_send\_\_sending\_to\_non-pid\_2\_\_depth\_2.spec} & 1201.36 & 0.06 \\
\texttt{firewall\_\_no\_pred\_called\_with\_zero\_\_depth\_2.spec} & 1201.34 & 599.79 \\
\texttt{main.spec} & 1175.42 & 599.75 \\
\texttt{main.spec} & 2.41 & 590.24 \\
\texttt{main.spec} & 1198.86 & 535.65 \\
\texttt{main.spec} & 4.21 & 510.54 \\
\texttt{main.spec} & 1.41 & 338.95 \\
\texttt{main.spec} & 1197.30 & 1.21 \\
\texttt{main.spec} & 122.81 & 1.23 \\
\texttt{main.spec} & 1197.98 & 1.28 \\
\texttt{main.spec} & 1190.65 & 1.27 \\
\texttt{main.spec} & 1176.27 & 1.24 \\
\texttt{main.spec} & 109.93 & 1.31 \\
\texttt{main.spec} & 1198.14 & 0.87 \\
\texttt{main.spec} & 3.75 & 1.03 \\
\texttt{main.spec} & 1200.95 & 1.27 \\
\texttt{main.spec} & 31.67 & 0.93 \\
\texttt{main.spec} & 104.48 & 1.17 \\
\texttt{main.spec} & 198.74 & 1.16 \\
\texttt{main.spec} & 1200.99 & 1.23 \\
\texttt{main.spec} & 1200.94 & 1.22 \\
\texttt{main.spec} & 13.05 & 1.27 \\
\texttt{main.spec} & 1191.12 & 1.25 \\
\texttt{main.spec} & 4.18 & 1.29 \\
\texttt{main.spec} & 15.97 & 1.28 \\
\texttt{main.spec} & 6.18 & 1.17 \\
\texttt{main.spec} & 1200.65 & 1.17 \\
\texttt{main.spec} & 1201.01 & 1.17 \\
\texttt{main.spec} & 1200.93 & 1.15 \\
\texttt{main.spec} & 1201.22 & 1.25 \\
\texttt{main.spec} & 1200.42 & 1.00 \\
\texttt{main.spec} & 1201.05 & 0.92 \\
\texttt{main.spec} & 8.71 & 1.06 \\
\texttt{main.spec} & 1200.59 & 0.80 \\
\texttt{main.spec} & 1200.86 & 0.88 \\
\texttt{main.spec} & 1201.09 & 0.98 \\
\texttt{main.spec} & 7.95 & 1.22 \\
\texttt{main.spec} & 188.37 & 0.98 \\
\texttt{main.spec} & 113.30 & 1.25 \\
\texttt{main.spec} & 1200.83 & 1.22 \\
\texttt{main.spec} & 1201.15 & 1.19 \\
\texttt{main.spec} & 1200.78 & 1.21 \\
\texttt{main.spec} & 1.00 & 1.04 \\
\texttt{main.spec} & 165.75 & 1.16 \\
\texttt{main.spec} & 1200.35 & 1.23 \\
\texttt{main.spec} & 5.99 & 1.24 \\
\texttt{main.spec} & 0.28 & 1.17 \\
\texttt{main.spec} & 1201.09 & 1.22 \\
\bottomrule
\end{longtable}
\normalsize

